YouTube over Google's QUIC vs Internet Middleboxes: A Tug of War between Protocol Sustainability and Application QoE

Middleboxes such as web proxies, firewalls, etc. are widely deployed in today's network infrastructure. As a result, most protocols need to adapt their behavior to co-exist. One of the most commonly used transport protocols, QUIC, adapts to such middleboxes by falling back to TCP, where they block it. In this paper, we argue that the blind fallback behavior of QUIC, i.e., not distinguishing between failures caused by middleboxes and that caused by network congestion, hugely impacts the performance of QUIC. For this, we focus on YouTube video streaming and conduct a measurement study by utilizing production endpoints of YouTube by enabling TCP and QUIC at a time. In total, we collect over 2600 streaming hours of data over various bandwidth patterns, from 5 different geographical locations and various video genres. To our surprise, we observe that the legacy setup (TCP) either outperforms or performs the same as the QUIC-enabled browser for more than 60% of cases. We see that our observation is consistent across individual QoE parameters, bandwidth patterns, locations, and videos. Next, we conduct a deep-dive analysis to discover the root cause behind such behavior. We find a good correlation (0.3-0.7) between fallback and QoE drop events, i.e., quality drop and re-buffering or stalling. We further perform Granger causal analysis and find that fallback Granger causes either quality drop or stalling for 70% of the QUIC-enabled sessions. We believe our study will help designers revisit the decision to enable fallback in QUIC and distinguish between the packet drops caused by middleboxes and network congestion.

==> Introduction.tex <==
\section{INTRODUCTION}
For performance and security reasons middleboxes are widely deployed in current network infrastructure. They offer benefits in terms of security (e.g., firewall, intrusion detection system), performance (e.g., proxies, load balancers) and bandwidth optimizers (e.g., WAN optimizer) and so on.   It is often speculated that that there are as many middleboxes as there are routers in the Internet~\cite{middlebox-more}. As a result, most protocols adapt their behaviour acknowledging the presence of middleboxes. For example, Google's QUIC protocol adapts to middleboxes that block QUIC traffic by falling back to TCP. If a server supports QUIC, the browser (chrome) would race a TCP connection with QUIC, whichever finishes first gets used for serving the request. In case, the connection fails QUIC is marked as broken for a time out duration of 5 minutes or decided by exponential backoff. The request then falls back to TCP.  

In this paper, we investigate the impact of adaptation behaviour of QUIC protocol in presence of middleboxes on its performance. For this, we focus on video streaming traffic as a majority i.e., $82\%$ Internet traffic is contributed by the video. Moreover  web traffic is mostly short lived, hence the impact of such fallback might not manifest. Video streaming  has become one of the most popular applications on the Internet where service providers like YouTube, Netflix are in high demand amongst the users. Google's QUIC protocol has gained a lot of popularity in recent years due to its benefits over TCP and has been largely adopted by Internet companies. As per cisco study, QUIC is being used by over $5\%$ of the top $10$ million websites\cite{ciscos}. QUIC offers many advantages, it allows (a) 0-RTT connection establishment, (b) improved congestion control, (c)
multiplexing without head-of-line blocking, (d) forward error correction and so on. Google proposed QUIC (Quick UDP Internet Connection) in the year $2013$ and implemented it on top of UDP as a new improved protocol at the application layer. Google delivers most of its Internet traffic over QUIC \cite{trafficq} that claims to reduce latency, page load time of websites. It also claims to reduce re-buffering in streaming YouTube videos. Google announced that the users experienced $30\%$ lesser re-buffering while streaming videos on YouTube\cite{quicd}. It also claims to improve the Quality of Experience (QoE) of the users. 

 

\iffalse
Recently, several studies have been conducted to understand the behaviour of DASH over transport layer protocols namely QUIC and TCP \cite{mondal2017candid,palmer2018quic,marx2020same}. For instance, in \cite{bhat2017not} authors tried to look at the DASH algorithm QoE performance for QUIC and TCP where both server and client were under controlled environment and also they stream shorter videos of around 5 min that are hosted on their different servers located at different locations. They observe that QUIC degrades the bitrate selection in some locations for the videos that are streaming over WiFi. In this work, we aim to compare the performance of QUIC over UDP with respect to TCP during video streaming using a specific web based streaming application, YouTube. The goal is to find out the performance QUIC protocols in varying bandwidth environments. For this we used the formula based QoE metric of \cite{mao2017neural} whose parameters are bitrate, bitrate variation and re-buffering. 


With additional benefits that QUIC enjoys, in this paper we aim to find out that whether QUIC always outperforms TCP in real network environment. Varying bandwidth a major concern in today's network. In this paper, We ask a few questions: (a) Whether QUIC always outperforms TCP irrespective of the changes on the network conditions. (b) If not, then what could be the possible reasons affecting the protocol performance. To answer these questions, we focus on video streaming over Youtube an internet application that is delivered via QUIC.
To the best of our knowledge, no prior work has looked at how QUIC and TCP behaves in varying bandwidth environments for application like YouTube. 
\fi


With additional benefits that QUIC enjoys, we expect to get better performance using QUIC than TCP in real network environment. For this, we set up a testbed to capture the browser traffic streamed from the YouTube server. We stream $1023$ videos over Youtube using both QUIC and TCP. We compute QoE of the videos using the formula specified Pensieve paper~\cite{mao2017neural}. We create a list of  $46$ videos and run them in multiple iterations. We choose videos from different genres such as news, entertainment shows, education videos, Indian talk shows, comedy shows, Stanford online lectures, British TV series (details are in Table.~\ref{video-details}). Each video has a duration of around $3600$ sec, hence our collected dataset is of around \textit{$36$ million} seconds in total. We played the videos under various bandwidth patterns (a) high bandwidth: when the bandwidth is above $640$ Kbps, we call it as high bandwidth, (b) low bandwidth: when it is below $640$ Kbps, we call it as low bandwidth, (c) dynamic bandwidth: when the bandwidth changes dynamically either dropping the bandwidth from high to low or suddenly increasing the bandwidth from low to high and so on in order to study the impact of bandwidth change over TCP and QUIC.  The videos were played across $5$ different geographical locations namely Delhi, Bangalore, Germany, Singapore and New York using Digital Ocean machines \cite{Do}. We collect the logs both at the application layer and at the network layer. We develop a chrome extension to download the application layer logs.
The application layer log contains HTTP request and responses. HTTP response  contains \textit{video playback} and \textit{streaming stat} details. The video playback information contains information about the segment requested, the time when the segment was requested and received, the quality or the itag of the requested segment and the total bytes of the requested segment. The streaming stat information contains the information about the video when it was actually played. The information like at real time `t', how much video was actually played called playback time `t1' of the video, the itag at which the video was played at time t1, buffer health tells about the amount of video already buffered at time t1. We also collect packet traces to get the network level exchanges.

From our experiments, we observed that the TCP either outperforms QUIC or performs the same as TCP in terms of QoE for most cases. We perform hypothesis testing to check the statistical significance of our observation that QUIC underperforms for most cases. We perform Welch's t-test across all the collected videos. We make our null hypothesis as QUIC is same as TCP and the alternate as the opposite.
%We conclud that the QoE obtained by these two protocols are statistically different from each other and are bandwidth agnostic. 
We found that for $20\%$ of all the videos these two protocols provide statistically similar QoE, for $41\%$ cases TCP performs better than QUIC and for $39\%$ cases QUIC performs better than TCP. Based on these observations, we further analyze and try to see whether our observations are dependent on any specific factors such as specific geographical location as in \cite{bhat2017not}, or specific video, backbone bandwidth etc. Hence, we formulate a set of research questions to understand the reasons behind such behaviour: (a) Does it depend on the bandwidth change pattern i.e. for various bandwidth patterns still the performance of QUIC suffers, (b) Does it depend on individual video i.e. when same video is played over both the protocols, does QUIC still underperform?, (c) Does it depend on different geographical locations i.e. across various geographical locations does QUIC's performance still suffer?, (d) Does backbone bandwidth play a role i.e., does backbone bandwidth disruption causes one protocol to perform better?, (e) Does individual QoE parameters show similar behaviour of QUIC underperforms for most cases?

We observe that our observation of QUIC underperforming is consistent across various bandwidth patterns, videos, locations, and individual QoE parameters. We also observe that backbone bandwidth does not play a role here. Hence, we take a further step and try to find out the root cause behind such behaviour. Note that to guard against middleboxes, QUIC falls back to TCP if a connection request fails.
Such a fallback behaviour does not differentiate between failure due to middleboxes and network congestion. In this paper, we claim that such blind fallback behaviour to co-exist with middleboxes impacts the performance  of QUIC.  We observe that under poor bandwidth, many such QUIC connections fall back to TCP. Due to the falback, QUIC faces additional performance impact in comparison to streaming the video over TCP only. Note that previous research observed that under high bandwidth both protocols perform similarly. Under fluctuating bandwidth, QUIC outperforms TCP because of its non-ambiguous ACK policy. The authors in this paper also observed that under variable bandwidth QUIC obtains better throughput than TCP. To the best of our knowledge, none of the papers investigated the impact of fallback on QUIC performance. 

To inspect, if our observations are statistically significant, we calculate cross correlation between fallback and application layer events such as quality drop and stalling. Note that an instance of fallback might not have an instant impact on either quality or the stalling as there is a buffer which has already been accumulated for. The impact of fallback might be faced after a certain time window when the buffer gets exhausted. Hence, we compute cross-correlation \cite{Cc} that uses a lag to compute to correlation. We observe that fallback and quality drop \& fallback and stalling are highly correlated with correlation coefficient between $0.4-0.9$ with a lag value of $90 sec$. Next, we investigate if there is causal relationship between fallback and application layer events.  We performed granger causal analysis \cite{Gc} for the same. We note that fallback indeed granger causes both quality drop and stalling with a significance level of less than 0.001.\\
The key contribution of this paper can be summarized as follows:
\begin{itemize}
    \item We inspect the adaptation behaviour of QUIC in presence of middleboxes on the performance of QUIC. For this, we conduct a measurement of the performance of QUIC and TCP by streaming YouTube videos under varying bandwidth conditions and $5$ different geographical locations. We collect logs of $1023$ videos that comprises of around \textit{$36$ million} seconds in total. We observe that QUIC underperforms compared to TCP for most cases. TCP either provides better QoE or same QoE as QUIC for $61\%$ cases.
    \item We discover that blind fallback behaviour of QUIC, that does not distinguish between failures caused by middleboxes and failures due to poor network bandwidth, causes performance degradation. In our measurements, we observe many fallback events under poor bandwidth. We find that there is a high correlation between fallback events and quality drop \& fallback events and stalling. Additionally, we observe that fallback granger causes both quality drop or stalling.
\end{itemize}
We believe that our work is the first step towards uncovering the issues created by fallback behaviour of QUIC. We believe QUIC designers should take a deeper look at the failures caused by middleboxes and network congestion and adapt accordingly.
The remainder of the paper is organised as follows. Section II describes the related work and some background knowledge followed by sections III that describes the experimental setup of this paper and then section IV, results and analysis followed by section V, looking under the hood.

% \subsection{Existing Literature and Limitations}

% \subsection{Contribution}

==> Performance_Analysis.tex <==
\section{PERFORMANCE ANALYSIS}
\textcolor{blue}{this section is very small, combine it with results and analysis section, give appropriate name}
In this section we will discuss about hypothesis testing we did to prove our observations statistically, followed by the research questions we asked in this work. 

\subsection{Hypothesis testing}
We have collected the data by running the youtube videos in realistic environment and then we did analysis. We looked at the QoE metrics for comparison and perform statistical testing on QoE of all the videos.
We also did two-tail test to check alternative hypothesis that when two protocols behave differently then which perform significantly better.
We begin our hypothesis testing by first calculating the single QoE value for each video for both QUIC and TCP which failed as discussed in section 4.4.2 and hence averaging is not a good approach for such cases where instantaneous changes are contributing the most in the observation.\\
We then calculate the instantaneous QoE for each video, the average bitrate, average bitrate variation and average stalling at every instant of time 't\textsubscript{k}' from the beginning at time 't\textsubscript{0}' till that time instant t\textsubscript{k} were calculated and this way we got multiple QoE values for one video for both TCP and QUIC. By using this approach even the smaller change in the QoE parameters was captured and can be used for comparison between QUIC and TCP.
Our Hypothesis results for all 500 videos are shown in Figure 4.

\begin{figure}[H]
  \centering
  \includegraphics[width=10cm,height=6cm]{images/histo_of_hypo_all.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{Hypothesis testing result of all the collected video}
          \label{example}
\end{figure}

Such observations led us to investigate further and we ask these questions: (1) \textit{does it depends on the bandwidth change patterns} that we are emulating in our experiment, (2) \textit{does it depends on the individual videos} such that every time the same video was played the one particular protocol performs always better, (3) \textit{does backbone bandwidth plays any role here} and, finally (4) \textit{QoE individual parameters show similar kind of behaviour or different behaviour}. We try to answer these questions in the next section.

==> extra.tex <==

%We start with the fallback experienced over the course of the experiments. Then we look at performance of TCP and QUIC in an exhausive fashion by varying bandwidth patterns, locations and so on. 

\iffalse
\textit{Fallback happening:}
Note that when we run a video specifying QUIC as the protocol, since the server is known to support QUIC, it will race a TCP connection with the QUIC connection, whichever finishes first is used for serving the request. However, if  this 0-RTT connection fails then it was assumed that the QUIC connection is broken for a timeout period determined by exponential backoff. Then the request falls back to TCP. In our case, we observe that under poor bandwidth many such QUIC connections fallback to TCP. For very low bandwidth, we observe continuous fallbacks throughout the video. 
\fi
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=14cm,height=7cm]{images/individual-scatter-plot.png}
%   \captionsetup{justification=centering,margin=2cm}
%          \caption{Instantaneous QoE value for a single video}
%           \label{fallback}
% \end{figure}



%With various enhancement that QUIC enjoys, one would expect gain a better performance using QUIC compared to TCP. However, our observations are the opposite. This led us to investigate further to see if this is due to any particular parameter or configurations that we have used. Hence, we  varied the parameters used and asked these questions: (1) \textit{does individual QoE parameters show similar kind of behaviour}, (2) \textit{does it depend on the bandwidth change patterns} that we are emulating in our experiment, (3) \textit{does it depend on geographical locations}, (4) \textit{does it depend on the individual videos}, and finally (5) \textit{does backbone network play any role here}. We answer these questions in next section.

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.3\textwidth}
%     \includegraphics[width=\textwidth]{increasing-bw.png}
%     \caption{increasing-bw.}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.3\textwidth}
%     \includegraphics[width=\textwidth]{decreasing-bw.png}
%     \caption{decreasing-bw.}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.3\textwidth}
%     \includegraphics[width=\textwidth]{sudden-6.png}
%     \caption{sudden bandwidth.}
%   \end{minipage}
% \end{figure}
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=14cm,height=7cm]{images/qoe-dist-tcpb.png}
%   \captionsetup{justification=centering,margin=2cm}
%          \caption{Distribution of QoE values for videos where TCP better than QUIC}
%           \label{fallback}
% \end{figure}

\iffalse
\begin{figure}[H]
  \centering
  \includegraphics[width=12cm,height=7cm]{images/histogram for entire videos.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{The percentage of videos where TCP and QUIC perform same and different in terms of QoE}
          \label{hypothesis-result}
          \vspace{-0.4cm}
\end{figure}

\fi
\iffalse
\begin{figure}
  \centering
  \includegraphics[width=10cm,height=6cm]{images/combine-scatter.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{Distribution of QUIC and TCP for combined 2 sample instances}
          \label{hypothesis-result}
          \vspace{-0.4cm}
\end{figure}
\fi

%This motivated us to plot the QoE distribution of QUIC and TCP performance for some $10$ sample videos. In Fig.~\ref{individual-para}(a) we can clearly see the difference in the performance of TCP and QUIC in terms of QoE in each individual video. For example, for video 1 the distribution of QUIC and TCP is almost same where the median values of both TCP and QUIC are $0.16$ and $0.15$ respectively whereas the 75th percentile of QUIC is $0.63$ and of TCP is $0.65$ which is slightly better than TCP. For video 7 the QoE of TCP is much better than QUIC also the median is high which is 0.86 for TCP and 0.58 for QUIC. The 75th percentile of TCP is also higher than QUIC i.e 0.82 for TCP and 0.59 for QUIC. For video 8 again the QoE of TCP is higher than QUIC and also the median which is 0.81 for TCP and 0.51 for QUIC.
%However, when we plotted the distribution of these these videos together in  Fig.~\ref{QoE-distribution}(b), we can no longer see the differences.
%see TCP becomes an winner. Even though for one video QUIC was winner and for the other TCP was the winner.
%we observed that the median of TCP is 0.41 which is higher than the median of QUIC which is 0.24. The 75th percentile of TCP was higher than QUIC i.e 0.57 for TCP and 0.29 for TCP. The 25th percentile of TCP is 0.39 and that of QUIC is 0.17 which is worser than TCP.
%Hence, we concluded that we should compute QoE of  each video individually.
\iffalse
\begin{figure}[H]
  \centering
  \includegraphics[width=11cm,height=7cm]{image-boxplot/1023_n_qoe.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{QoE distribution across all $1023$ videos}
         \vspace{0.2cm}
          \label{QoE-distribution}
\end{figure}
\fi
\iffalse
\begin{figure}[t]
  \centering
  \includegraphics[width=14cm,height=7cm]{images/fallback with annonate.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{Number of bytes transferred over TCP and QUIC, while specifying QUIC as the protocol for streaming a video}
          \label{fallback}
          \vspace{-0.4cm}
\end{figure}

\begin{figure}[H]
  \centering
  \includegraphics[width=14cm,height=7cm]{images/cdf-fallback-tcp.pdf}
  \captionsetup{justification=centering,margin=2cm}
         \caption{Percentage of fallback i.e., percentage of bytes transferred over TCP for various bandwidth patterns}
          \label{fallback-percent}
          \vspace{-0.4cm}
\end{figure}
\fi
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=12cm,height=7cm]{images/v21_slot-13_quic.csv_qual_graphs.png}
%   \captionsetup{justification=centering,margin=2cm}
%          \caption{Stall vs Real time graph}
%           \label{example}
% \end{figure}
Initially, we observed that our institute's firewall blocks all QUIC traffic, hence even though we specified to run over QUIC it actually ran over TCP protocol. We understood that this is due to fallback option supported by QUIC to sustain across middleboxes. Next, we made an exception in the firewall rules and allowed QUIC traffic. 


\subsection{Cross Correlation}
\label{cc-about}
Cross Correlation is a measure of similarity between the two signals or variables say A and B. It is measured through the displacement of one signal relative to other signal. In Fig.~\ref{cross-corr-ex}(a) there are two signals, signal A and signal B and they differ from each other by some shift say \textit{l} along the x axis. Cross correlation function does the shifting of one signal in both directions such that the maximum matching between the two signals can be obtained. Then it returns the correlation value of similarity between two signals and lag value at which this maximum correlation is observed. We have implemented it using xcorr() function of MATLAB.
\begin{figure}[t]
\subfloat[Example to showcase how cross correlation works]{\includegraphics[width = 3.3in]{images/sin-cos signal-new1.jpg}}
\subfloat[QUIC and TCP having different bitrate/quality throughout the video at varying bandwidth for a sample video ]{\includegraphics[width = 3.3in]{images/dynamic-low.png}}
\caption{Cross correlation example, TCP, QUIC quality for a sample video}
\label{cross-corr-ex}
\vspace{-0.4cm}
\end{figure}

\iffalse
\begin{figure}[H]
  \centering
  \includegraphics[width=12cm,height=3cm]{images/sin-cos signal-new1.jpg}
  \captionsetup{justification=centering,margin=2cm}
  \vspace{-0.2cm}
         \caption{Example to showcase how cross correlation works}
          \vspace{-0.6cm}
          \label{cross-corr-ex}
\end{figure}
\fi
\subsection{Granger Causality}
It a hypothesis testing which is used for predicting/forecasting one time series using another time series. Granger causality is a causal model for a time series data and it is used for finding out the cause and effect relationship between the two variables where one variable is the cause and the another variable is an effect of that cause. We have linear Granger Causal model that internally uses linear regression. It creates two models say model 1 and model 2. Model 1 is used for predicting the X present values based on lag past values X series and model 2 is also used for predicting the present value of X based on the lag past values of X and Y both series. It is said that Y granger causes X (Y->X) if the prediction error of model 2 is significantly smaller than model 1 prediction error. So, the null hypothesis for granger causality test is \textit{'Y does not granger causes X'} and alternative hypothesis is \textit{'Y granger causes X'}. There are few prerequisite for performing the Granger Causality test that is the data needs to be stationary. To check whether the data is stationary or not a test called KPSS (Kwiatkowski–Phillips–Schmidt–Shin) test \cite{Kpss} and ADF (Augmented Dickey-Fuller) test \cite{adf} is used and if data is found to be non-stationary then it is transformed to stationary data by differentiating it. If after first order differentiation the data is non-stationary, the second order differentiation is performed and if the test again fails then the granger causality test is not performed.





\subsection{Background on Statistical Analysis}
\subsection{Hypothesis Testing}
Hypothesis testing is a testing to prove a statement or an hypothesis that is yet to be proven. There are two hypothesis one is null hypothesis (H\textsubscript{0}) which is to be proven statistically and it is an assertion we believe in. Another is alternative hypothesis (H\textsubscript{1}) which is a negation of null hypothesis. When we assume that our null hypothesis is that two populations have equal means we perform two-tail test and when we assume that one population has greater mean than other then we perform one-tail test. We have used Welch t-test on our dataset. Welch t-test has an assumption that the two variables or populations are normally distributed with unequal variances. We use the ttest2() function of MATLAB to perform the welch t-test which returns the h value and if h=0 we say the null hypothesis cannot be rejected at 5\% significance level and h=1 says that the null hypothesis can be rejected at 5\% significance level. The significance level is also known as probablity level of significance.

% In our work we first try to observe the behavior of QUIC and TCP by using video quality and real time graphs and so in order to state our observations statistically we performed Welch's ttest on QoE values with the null hypothesis as \textit{'QUIC will perform same as TCP'} and alternative hypothesis as \textit{'QUIC and TCP will perform differently'} with a significance level alpha as 0.05.
%We observe from Fig~\ref{hypothesis-location} that in cases of Bangalore and Germany the performance of QUIC was better than TCP for majority cases. However, for Delhi and New York the performance of TCP was better than QUIC for majority cases. Hence, we cannot conclude that performance of QUIC depends on a specific geographical location.

%Fig.~\ref{qoe-location} shows the distribution of QoE values for $5$ sample videos over these locations.  Fig.~\ref{qoe-location}(a) shows QoE distribution at Delhi. For example,  for video 1 the median of TCP is higher than QUIC i.e for TCP it is $0.57$ and for QUIC it is $0.42$. TCP is worst at 25th percentile and is better at 75th percentile that TCP is $0.71$ and QUIC is $0.59$.
%For video 2 the QoE distribution of TCP and QUIC is very low and the median of QUIC is better than TCP i.e 0.26 for QUIC and 0.12 for TCP whereas the 75th percentile is same for both.
%For video 3 the median of TCP is better than QUIC i.e. 0.76 for TCP and 0.51 for QUIC. The 75th percentile is again higher for TCP i.e 0.82 and 0.61 for QUIC. For video 4 the median and 25th percentile of TCP and QUIC is almost similar but the 75th percentile of TCP is more than QUIC i.e., 0.71 for TCP and 0.57 for QUIC.
%For video 5, the median of TCP is higher than QUIC i.e 0.54 for TCP and 0.44 for QUIC. Also the 25th percentile of TCP is more than QUIC and the 75th percentile as well i.e, 0.57 for TCP and 0.51 for QUIC. 
%Fig.~\ref{qoe-location}(b) shows QoE distribution at Bangalore. For example,  or video 1 the median of TCP i.e 0.43 is higher than median of QUIC i.e 0.34.
%The 75th percentile of TCP is higher than QUIC i.e 0.51 for TCP and 0.45 for QUIC but at 25th percentile the TCP perform worse than QUIC i.e. 0.23 for QUIC and 0.19 for TCP. For video 2 the QoE distribution of both the protocols are low but the median of QUIC i.e 0.21 is higher than median of TCP i.e 0.06. For video 3 the median of QUIC is much higher than TCP i.e it is 0.66 for QUIC and 0.19 for TCP. The 75th percentile of QUIC is also higher which is 0.72 than TCP which is 0.55. At 25th percentile the QUIC is again higher i.e 0.39 than TCP i.e 0.18. For video 4 the median of QUIC is higher than TCP i.e 0.76 and 0.51 for QUIC. Foe video 5 again the QUIC median is much higher than TCP i.e 0.64 for QUIC and 0.26 for TCP. Also the 75th percentile and 25th percentile are higher for QUIC which clearly states that they are different. 
%Fig.~\ref{qoe-location}(c) shows QoE distribution at New york. For example,  for video 1 the median of TCP is slightly higher than median of QUIC but QUIC perform worse at 25th percentile i.e 0.44 for TCP and 0.30 for QUIC. 
%For video 2 the median of TCP was higher than QUIC i.e 0.34 for TCP and 0.21 for QUIC. The QUIC perform worse at 25th percentile i.e it is 0.20 for TCP and 0.14 for QUIC. For video 3 the median of TCP and QUIC are almost similar but the 75th percentile of TCP was better than QUIC i.e., 0.47 for QUIC and 0.36 for TCP. For video 4 the QoE distribution of QUIC and TCP is very low and the 75th percentile of QUIC is worser than TCP i.e., 0.25 for TCP and 0.18 for QUIC. For video 5 the median of QUIC is higher than TCP i.e 0.58 for QUIC and 0.49 for TCP. Also the 75th percentile of QUIC is higher than TCP i.e 0.70 for QUIC and 0.56 for TCP. 
%Fig.~\ref{qoe-location}(d) shows QoE distribution at Germany. For example, where for video 1 the median of QUIC is higher than TCP i.e 0.65 for QUIC and 0.43 for TCP but the 75th percentile of TCP is higher than QUIC i.e 0.84 for TCP and 0.70 for QUIC. 
%For video 2 the median of QUIC is slightly higher than TCP but the QUIC has better 25th percentile than TCP i.e. 0.37 for QUIC and 0.30 for TCP. For video 3 the median of QUIC is again higher than TCP i.e 0.45 for QUIC and 0.36 for TCP. Also the QoE distribution of TCP is quite dispersed whereas it is skewed for QUIC. There was a huge difference between the 25th percentile of QUIC and TCP where QUIC has better 25th percentile i.e it is 0.08 for TCP and 0.39 for QUIC. For video 4 the distribution of two protocol looks same where the QUIC 75th percentile is slightly more than TCP i.e 0.34 for TCP and 0.36 for QUIC. For video 5 the QoE distribution of QUIC is better than TCP and is quite close to 1. The median of QUIC which is 0.88 is higher than TCP which is 0.64.
%Fig.~\ref{qoe-location}(e) shows QoE distribution at Singapore. For example, for video 1 the median of QUIC is 0.44 higher than median of TCP i.e 0.18. Also the 75th percentile and the 25th percentile of QUIC is also higher than TCP. 
%For video 2 the median of TCP is higher than QUIC i.e 0.69 for TCP and 0.40 for QUIC. The 75th percentile is also higher for TCP which is 0.76 for TCP and 0.45 for QUIC. For video 3 the median of QUIC is higher than TCP i.e 0.43 for QUIC and 0.26 for TCP. For video 4 the median of TCP was higher than QUIC i.e 0.77 for TCP and 0.51 for QUIC but the 25th percentile of QUIC is high which is 0.46 for QUIC and 0.28 for TCP. For video 5 the distribution of both TCP and QUIC is low but the median of TCP is slightly higher than TCP where it is 0.32 for TCP and 0.26 for QUIC. The 75th percentile of TCP is also slightly higher than QUIC i.e 0.35 for TCP and 0.29 for QUIC.


% \begin{figure}[t]
% \subfloat[QoE of QUIC vs TCP for Delhi]{\includegraphics[width = 2.2in]{image-boxplot/delhi.png}}
% \subfloat[QoE of QUIC vs TCP for Bangalore]{\includegraphics[width = 2.2in]{image-boxplot/bangalore.png}} 
% \subfloat[QoE of QUIC vs TCP for New York]{\includegraphics[width = 2.2in]{image-boxplot/newyork.png}}\\
% \subfloat[QoE of QUIC vs TCP for Germany]{\includegraphics[width = 2.2in]{image-boxplot/germany.png}}
% \subfloat[QoE of QUIC vs TCP for Singapore]{\includegraphics[width = 2.2in]{image-boxplot/singapore.png}} 
% \caption{QoE distribution at  different geographical locations for $5$ sample videos}
% \label{qoe-location}
% \vspace{-0.4cm}
% \end{figure}



\iffalse
\begin{figure}[H]
  \centering
  \includegraphics[width=12cm,height=6cm]{images/geographical-loc-graph-14jan.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{The percentage of videos where TCP and QUIC perform same and different in terms of QoE  across different geographical locations}
          \label{hypothesis-location}
          \vspace{-0.4cm}
\end{figure}
\fi

%We show the results of hypothesis testing in Fig.~\ref{qoe-hypothesis-same-video}(b).  We have the similar observation here also that sometimes TCP performs better and sometimes QUIC and hence we again cannot conclude anything.

% \begin{figure}
% \subfloat[QoE of QUIC vs TCP]{\includegraphics[width = 2in]{images/QoE-individual.pdf}} 
% \subfloat[Average bitrate of QUIC vs TCP]{\includegraphics[width = 2in]{images/Avg_bitrate-individual.pdf}}
% \subfloat[Average bitrate variation of QUIC vs TCP]{\includegraphics[width = 2in]{images/Avg_bitrate_variation-individual.pdf}}\\
% \subfloat[Average stall of QUIC vs TCP]{\includegraphics[width = 2in]{images/Avg_stall-individual.pdf}} 
% \caption{The analysis of videos where TCP$>$QUIC and QUIC$>$TCP for same video running multiple times}
% \label{cross-corr}
% \end{figure}
\iffalse
\begin{figure}
  \centering
  \includegraphics[width=12cm,height=7cm]{image-boxplot/n_qoe_slots.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{QoE distribution of same video ran at multiple times}
          \label{qoe-same-video}
          \vspace{-0.4cm}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=12cm,height=7cm]{images/slot-wise-graph-new.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{The percentage of videos where TCP$>$QUIC and QUIC$>$TCP for same video running multiple times}
          \label{hypothesis-same-video}
          \vspace{-0.4cm}
\end{figure}
\fi
% \subsection{Does Backbone Network Play A Role?}
% To answer this question, we ran the videos without throttler. We saw that there were no quality variation and no stalling events in the entire video. Moreover, it was played at high quality $720$p all throughout the video. Hence, we conclude that backbone network does not play a role here.
\iffalse
\begin{figure}[H]
  \centering
  \includegraphics[width=12cm,height=6cm]{images/no throttler.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{When TCP and QUIC videos were played without a throttler}
          \label{no-throttler}
          \vspace{-0.4cm}
\end{figure}

 \fi


\iffalse
Note that when we run a video specifying QUIC as the protocol, since the server is known to support QUIC, it will race a TCP connection with the QUIC connection, whichever finishes first is used for serving the request. However, if  this $0$-RTT connection fails then it was assumed that the QUIC connection is broken for a timeout period determined by exponential backoff. Then the request falls back to TCP. In our case, we observe that under poor bandwidth many such QUIC connections fallback to TCP. For very low bandwidth, we observe continuous fallbacks throughout the video.  Fig.~\ref{fallback} shows the bytes transferred over both TCP and QUIC. The figure shows the heavy presence of TCP packets although the video was run specifying QUIC as the protocol. This phenomenon is called as fallback and the figure shows there are several such fallback events.
\fi


 

% \begin{figure}[H]
%   \centering
%   \includegraphics[width=12cm,height=7cm]{images/v21_slot-13_quic.csv_qual_graphs.png}
%   \captionsetup{justification=centering,margin=2cm}
%          \caption{Stall vs Real time graph}
%           \label{example}
% \end{figure}
\iffalse
\begin{figure}[H]
  \centering
  \includegraphics[width=14cm,height=7cm]{images/bandwidth-fallback_plot.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{Number of bytes transferred over TCP and QUIC, while specifying QUIC as the protocol for streaming a video}
          \label{fallback-under}
          \vspace{0.4cm}
\end{figure}
\fi


% \begin{table}[H]
% \begin{tabular}{|l |l|l|}
% \hline
% \textbf{QUIC} & \textbf{Quality drop} & \textbf{Rebuffering} \\ \hline
% \textbf{Bandwidth drop + No-fallback} & 40\% & 50\% \\ \hline
% \textbf{Bandwidth drop + Fallback} & 70\% & 100\% \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[H]
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{TCP} & \textbf{Quality Drop} & \textbf{Rebuffering} \\ \hline
% \textbf{Bandwidth drop} & 100\% & 100\% \\ \hline
% \end{tabular}
% \end{table}
%found out the configuration parameters through which the fair comparison can be done between QUIC and TCP and also in order to find out how QUIC and TCP performs they automate the process of generating network traffic on servers of TCP and QUIC in desktop and mobile environment. They also try to understand how QUIC evolved over time and how its performance improved with time.
%One of their observation says that QUIC outperforms TCP in scenarios with fluctuating bandwidth. We in this paper on the other hand tried to observe QUIC and TCP in similar scenarios where there are fluctuations in bandwidth in case of video streaming application like YouTube that uses very optimized version of QUIC. 
% we first consider five randomly selected session pairs from each of the five bandwidth patterns and observe QoE distributions across those session pairs. Fig.~\ref{qoe-bandwidth-samples} shows the results. For increasing and decreasing bandwidth shapers (Figs.~\ref{qoe-bandwidth-samples}(a) and \ref{qoe-bandwidth-samples}(a)), we do not see any significant difference ($p>0.05$) between QUIC-enabled streams and TCP streams in terms of perceived video QoE over YouTube. However, for dynamic high bandwidth shaper, we see that TCP streams work better for sessions S2 and S4 ($p<0.05$), whereas QUIC-enabled streams outperform TCP streams in S5 ($p<0.05$). Interestingly, for dynamic low bandwidth, TCP streams work better for S1, S3, and S5, whereas for dynamic very low bandwidth, QUIC-enabled streams suffer for S1, S4, and S5. However, there are some instances when QUIC-enabled streams perform better than TCP streams. 

% To analyze further,
% Fig.~\ref{qoe-bandwidth-samples} shows distribution of QoE for $5$ sample videos for each bandwidth. Fig.~\ref{qoe-bandwidth-samples}(a) shows QoE distribution of increasing bandwidth pattern. For video 1 we can see the median of QUIC which is 0.24 is higher than the TCP which is 0.15. For video 2 the TCP median which is 0.22 is higher than QUIC median which is 0.16 and also the the 25th and 75th percentile. 
% \iffalse
% For video 3 the TCP median is worst than QUIC median where TCP median is 0.07 and QUIC median is 0.26. Though the 75th percentile of TCP is higher which is 0.67 for TCP and 0.62 for QUIC. For video 4 the two distribution looks same where there median and 25th percentile has a slight difference. For video 5 the TCP median i.e 0.48 is higher than QUIC median i.e 0.40, the 75th percentile of TCP is also slightly higher i.e 0.84 than QUIC i.e. 0.80.
% \fi
% Fig.~\ref{qoe-bandwidth-samples}(b) shows QoE distribution of decreasing bandwidth pattern. For all $5$ sample videos, the QoE distribution for both TCP and QUIC are high i.e close to 1. As expected for high bandwidth both the protocols behave almost same and higher QoE can be experienced.
% Fig.~\ref{qoe-bandwidth-samples}(c) shows QoE distribution of dynamic-high bandwidth pattern. For video 1 the overall QoE distribution of both the protocols are high i.e close to 1. The median of TCP is slightly better than QUIC i.e, 0.95 for TCP and 0.91 for QUIC. 
% %At 25th percentile, the TCP again has better QoE whereas at 75th percentile both has same QoE.
% For video 2 the TCP QoE distribution is much higher than QUIC and also the distribution is high and close to 1. The median of QUIC is 0.53 and of TCP is 0.92 which is again much higher than QUIC. 
% %Similarly the TCP 25th and 75th percentiles are higher than QUIC. 
% For video 3 the two protocols TCP and  QUIC have almost similar QoE distribution. 
%For Video 4, the TCP median i.e 0.51 is higher than QUIC median i.e 0.30. Also the QUIC 25th and 75th percentile is also worser than TCP. For video 5, from distribution plot we can see that the QoE is very dispersed and is not centered around the median for both TCP and QUIC. The median of QUIC here is more than TCP which is 0.81 for QUIC and 0.61 for TCP. The 75th percentile of TCP is also worser than QUIC which is 0.79 for TCP and 0.94 for QUIC.
%Here we observe that in increasing bandwidth, the two protocols behave quite differently in the beginning when the bandwidth was low whereas this was not observed in decreasing bandwidth pattern since the bandwidth was sufficient and so the two protocols behave similarly. Overall, we observed that high bandwidth, we mostly experience higher QoE for most of the videos. As high bandwidth allows the buffer to get filled a constant rate to avoid stalling.

%Fig.~\ref{qoe-bandwidth-samples}(d) shows QoE distribution of dynamic-low bandwidth pattern. For example, for video 1, the QoE distribution of TCP is higher than QUIC that is close to $1$. The median of TCP is $0.79$ much higher than median of QUIC which is 0.46. %Similarly the 25th and 75th percentile of TCP is much more for TCP than QUIC.
%For video 2, the median of TCP is much worser than QUIC where the TCP median is 0.22 and QUIC median is 0.64. Also the distribution of QoE for TCP is tightly clustered around the median whereas in QUIC it is spread out. The 75th percentile of QUIC is much more higher than TCP i.e 0.93 for QUIC and 0.45 for TCP. For video 3 the QoE distribution of both TCP and QUIC is low but the median of TCP i.e 0.24 is higher than QUIC which is 0.1. 
%Also the 75th percentile of TCP is 0.26 higher than QUIC that is 0.13. For video 4, we can see that the median of TCP and QUIC are almost same but 75th percentile of QUIC i.e 0.35 is higher than TCP i.e 0.29. For video 5 the QUIC QoE distribution is worst than TCP. Also the median of TCP is higher which is 0.33 than that of QUIC which is 0.17.  
%Fig.~\ref{qoe-bandwidth-samples}(e) shows QoE distribution of dynamic-very-low bandwidth pattern. For video 1 the TCP QoE distribution is higher than QUIC where the median of TCP is also high ie. $0.79$ for TCP and $0.59$ for QUIC. The 75th percentile also has a huge difference such that TCP is $0.90$ and QUIC is $0.63$. 
%For video 2 the overall QoE distribution for both TCP and QUIC is high, but the median of QUIC is slightly higher than TCP i.e 0.89 for QUIC and 0.82 for TCP. For video 3 the QoE distribution of QUIC is much more dispersed than TCP. Also the QUIC median i.e 0.69 is higher than TCP median i.e. 0.57. The 75th percentile of QUIC is also much higher than TCP i.e for QUIC it is 0.92 and for TCP it is 0.59. 
%For video 4, the median of TCP i.e 0.54 is higher than median of QUIC i.e 0.44. The 75th percentile of TCP is 0.57 slightly higher than QUIC which is 0.51. For video 5, the median of TCP is much higher than QUIC median i.e 0.89 for TCP and 0.64 for QUIC. Also there is a huge difference in the 75th percentile such that TCP has 0.91 and QUIC has 0.69.

%Additionally, we observe that in dynamic very low bandwidth since the bandwidth was very low most of the videos was played at minimum quality i.e at $144$p. In this case, the instances of quality drops are very less as there are no other quality options. Instead, we observe more rebuffering events. For dynamic low bandwidth, as there is a scope of quality drop to counter for poor bandwidth, there are more quality drop events along with rebuffering events. 
 
%  We show the results of hypothesis testing in Fig.~\ref{hypothesis-bandwidth-location}(a).  We observe that for increasing-bandwidth pattern, QUIC  either outperforms or performs the same as TCP for more than  $80$\% cases. Similarly, for decreasing-bandwidth, both QUIC and TCP perform the same for roughly $70$\% cases. At dynamic-high bandwidth, both TCP and QUIC showed similar QoE for $44$\% cases. Here, QUIC outperformed TCP for slighly more cases than TCP (TCP 28\% cases, QUIC 30\% cases).  For dynamic-low bandwidth, $21$\% of the cases the QoE of QUIC and TCP came out to be same and for the remaining $79$\% the QoE of QUIC and TCP was different. Here, TCP outperformed QUIC for a slightly more number of cases (TCP $41$\%, QUIC $39$\%). For dynamic-very-low bandwidth, $11$\% of the time the QoE of QUIC and TCP came out to be same and for the remaining $89$\% the QoE of QUIC and TCP was different. Here, TCP outperformed QUIC for more number of cases (TCP $50$\%, QUIC $35$\%).  Hence, we conclude that at lower bandwidths (dynamic-low and dymanic-very-low), QUIC starts to perform worser than TCP. Hence, TCP becomes an winner for most times. 


% \begin{figure}[H]
%   \centering
%   \begin{minipage}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth]{images/bandwidth_hypo_graphs.png}
%     \caption{shows the result of hypothesis testing for different bandwidth patterns. }
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth]{images/geographical_loc_graph.png}
%     \caption{shows the hypothesis result of different geographical locations}
%   \end{minipage}
% \end{figure}

% \begin{figure}[t]
% \subfloat[QoE of QUIC vs TCP for increasing bandwidth]{\includegraphics[width = 2in]{image-boxplot/increasing.png}}
% \subfloat[QoE of QUIC vs TCP for decreasing bandwidth]{\includegraphics[width = 2in]{image-boxplot/decreasing.png}} 
% \subfloat[QoE of QUIC vs TCP for dynamic-high bandwidth]{\includegraphics[width = 2in]{image-boxplot/dynamic-high.png}}\\
% \subfloat[QoE of QUIC vs TCP for dynamic-low bandwidth]{\includegraphics[width = 2in]{image-boxplot/dynamic-low.png}}
% \subfloat[QoE of QUIC vs TCP for dynamic-very-low bandwidth]{\includegraphics[width = 2in]{image-boxplot/dynamic-very-low.png}} 
% \caption{QoE distribution across different bandwidth patterns}
% \label{qoe-bandwidth-samples}
% \vspace{-0.6cm}
% \end{figure}
\iffalse
\begin{figure}[t]
  \centering
  \includegraphics[width=12cm,height=6cm]{images/bandwidth_hypo_graphs_new.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{The percentage of videos where TCP and QUIC perform same and different in terms of QoE across different bandwidth patterns }
          \label{hypothesis-bandwidth}
          \vspace{-0.4cm}
\end{figure}
\fi

%For the session pairs S1, S2, S4 and S9, we see that the distribution of average stall for TCP streams and QUIC are better than the distribution of average bitrate and average bitrate variation. The median of both TCP and QUIC in case of average bitrate and average bitrate variation is also very low whereas of average stall it is slightly better. For video 3 the distribution of average bitrate variation is worser than the distribution of average bitrate and average stall. In case of average stall the TCP distribution is very poor where the median of QUIC is much higher than that of TCP i.e 0.09 for TCP and 0.31 for QUIC. On the other hand for the same video in case of average stall the median of TCP was better than QUIC i.e 0.37 for TCP and 0.20 for QUIC. In case of video 5 for all three distributions namely average bitrate, average bitrate variation and average stall, the TCP is better than QUIC. For video 6 for average bitrate distribution of QUIC is much higher than TCP. The median of QUIC is 0.95 which is much higher than median of TCP i.e 0.35. The avergae bitrate variation distribution of QUIC and TCP is worst than other two parameters distribution whereas for average stall disribution the QUIC median is again higher than TCP. For video 7 the median of TCP is much higher than QUIC for the distribution of all three parameters. For video 8 the average bitrate variation distribution for both TCP and QUIC is worst close to 0. For average bitrate the median of QUIC is very close to 0 thus worst than TCP. For average stall the QUIC median is much higher than TCP. For video 10, the QUIC is better for average bitrate, average bitrate variation and average stall but the distribution of average bitrate variation is worst for both TCP and QUIC which is close to $0$.

%We now perform hypothesis testing on individual parameters of QoE formula i.e., average bitrate, average bitrate variation and average stalling. 
\iffalse
\begin{figure}
  \centering
  \includegraphics[width=10cm,height=6cm]{images/qoe_parameter_new.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{The percentage of videos where TCP and QUIC perform same and different across different QoE parameters}
          \label{hypothesis-individual-qoe}
          \vspace{-0.4cm}
\end{figure}
\fi
We next look at the instances of fallbacks over months. Though we had collected the dataset for about 1 year, we have the network level packet traces only for past 5 months.  Fig.~\ref{} shows the CCDF of fallback \% over 5 months namely September, October, November, December and January. We noticed significant fallback across all months. Interestingly, we observe that $40$\% times $20$\% or more bytes are transferred over TCP for October and January. Whereas, for September, November, and December $40$\%  times $56$\% , $65$\%, and $66$\% or more bytes transferred over TCP respectively. On further check, we noticed that we mostly collected data at DL during October and January, whereas during September, November and December we focused mostly on DVL. This corroborates with our previous observation that lower the bandwidth higher are the instances of fallback.

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}
There are number of studies on performance comparison of QUIC and TCP ~\cite{kakhki2017taking, quicker, palmer2018quic, wolsing2019performance, seufert2019quic, biswal2016does, dissecting, carlucci2015http, das2014evaluation, megyesi2016quick, yu2017quic}. Most studies suggest that QUIC outperforms TCP in terms of web browsing. However, there are conflicting claims about video streaming performance~\cite{kakhki2017taking, quicker}. This motivates us to analyze the performance of QUIC for video streaming traffic. Hence, we set up a testbed and conducted a few initial measurements. We play a video twice once with QUIC and then with TCP. We looked at the packet level trace to findout if indeed QUIC was being used when we run the video with QUIC protocol. Initially, we observed that our institute's firewall blocks all QUIC traffic, hence even though we specified to run over QUIC it actually ran over TCP protocol. We understood that this is due to fallback option supported by QUIC to sustain across middleboxes. Next, we made an exception in the firewall rules and allowed QUIC traffic. However, this time we had an interesting observation that there are mix of TCP and QUIC packets. This leads us to investigate further since this time our firewall was no longer blocking QUIC traffic. We analyzed the reason for this and found out that it is the poor bandwidth that causes unnecessary fallbacks to happen. Next, we ask this question, how do these unnecessary fallbacks impact QUIC's performance. To answer the same, we conduct a large scale measurement study of running over $1000$ videos in a span of $2$ years over various bandwidth patterns and $5$ different geographical locations. 

\iffalse
Hence, we conducted a large scale measurement to We observe that the two protocols were running at different qualities throughout the video as shown in Fig.~\ref{cross-corr-ex}{b}. As discussed in the previous section, we 

The motivation for this work comes from the widespread adoption of QUIC and from its increased popularity among the network research community. From the earlier research work, some researchers claimed that QUIC performs overall better than TCP at low bandwidth for loading a web page \cite{biswal2016does} and so this motivates us to understand how QUIC will perform for longer YouTube videos under varying bandwidth i.e not only on low bandwidth but also a bandwidth that is varying with time. YouTube also has a very optimized version of QUIC which is completely black box and needs to be examined. For this, we conducted a small experiment where vary the bandwidth using network emulator tool mahimahi while streaming an YouTube video and  collect  logs. We observe that the two protocols were running different qualities throughout the video as shown in Fig.~\ref{cross-corr-ex}{b}. Also, we know that network has a lot of randomness that might affect the overall observation. Thus, this further motivates us to collect the larger dataset to state our observations statistically and to understand which protocol performs better in which environmental condition and also to avoid any biasness. Prior works claimed that QUIC outperformed TCP and where some other research work claimed that QUIC and TCP perform the same but none of the researcher did the root cause analysis for those observations about why particular protocol performs better or poor and this motivates us to explore in more detail the root cause behind such behaviour of these two protocols. \textcolor{blue}{Expand the limitations of prior work in more concrete terms here and give references}

\begin{figure}[H]
  \centering
  \includegraphics[width=10cm,height=5cm]{images/dynamic-low.png}
  \captionsetup{justification=centering,margin=2cm}
         \caption{QUIC and TCP having different bitrate/quality throughout the video at varying bandwidth}
         \vspace{-0.2cm}
          \label{tcp-quic-ex}
          \vspace{-1cm}
\end{figure}
\fi
